Inverse Risk-Sensitive Reinforcement Learning

We address the problem of inverse reinforcement learning in Markov decision processes where the agent is risk-sensitive. In particular, we model risk-sensitivity in a reinforcement learning framework by making use of models of human decision-making having their origins in behavioral psychology, behavioral economics, and neuroscience. We propose a gradient-based inverse reinforcement learning algorithm that minimizes a loss function defined on the observed behavior. We demonstrate the performance of the proposed technique on two examples, the first of which is the canonical Grid World example and the second of which is a Markov decision process modeling passengers' decisions regarding ride-sharing. In the latter, we use pricing and travel time data from a ride-sharing company to construct the transition probabilities and rewards of the Markov decision process.

==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = 2017tac
# put the names of figure files here.  include the .eps
#figures =
# if no references, run "touch latexfile.bbl; touch referencefile.bib"
# or delete dependency in .dvi and tarball sections
referencefile = 2017tacrefs

TEX = pdflatex

# support subdirectories
VPATH = Figs

# reruns latex if needed.  to get rid of this capability, delete the
# three lines after the rule.  Delete .bbl dependency if not using
# BibTeX references.
# idea from http://ctan.unsw.edu.au/help/uk-tex-faq/Makefile
$(latexfile).pdf : $(figures) $(latexfile).tex
#$(latexfile).dvi : $(figures) $(latexfile).tex $(latexfile).bbl
	while ($(TEX) $(latexfile) ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


# keep .eps files in the same directory as the .fig files
#%.eps : %.fig
#	fig2dev -L eps $< > $(dir $< )$@

#$(latexfile).pdf : $(latexfile).ps
#	ps2pdf $(latexfile).ps $(latexfile).pdf

#pdf : $(latexfile).pdf

#$(latexfile).ps : $(latexfile).dvi
#	dvips $(latexfile)

#ps : $(latexfile).ps

# make can't know all the sourcefiles.  some file may not have
# sourcefiles, e.g. eps's taken from other documents.
#$(latexfile).tar.gz : $(figures) $(latexfile).tex $(referencefile).bib
#	tar -czvf $(latexfile).tar.gz $^

#tarball: $(latexfile).tar.gz

cpall:
	make; skim $(latexfile).pdf

clean:
	#rm $(latexfile).aux $(latexfile).log $(latexfile).pdf
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk

fixpdf:
	gs -dSAFER -dBATCH -dNOPAUSE  -sDEVICE=pdfwrite -sOutputFile=fixed.pdf $(latexfile).pdf

mpdf:
	$(TEX) $(latexfile).tex; skim $(latexfile).pdf

mbib:
	$(TEX) $(latexfile).tex; bibtex $(latexfile); $(TEX) $(latexfile).tex; $(TEX) $(latexfile).tex; skim $(latexfile).pdf


==> proofThmQ_old.tex <==

%\begin{proof}
   % Let $L=\max_\theta\{L_y(\theta),L_\theta\}$. We re-write our $Q$--update equation as follows:
   % \begin{align}
   %     Q_{t+1}(x,a,\theta)=&\left( 1-\frac{\alpha_t}{\alpha}
   %     \right)Q_t(x,a,\theta)\notag\\
   %     &\quad+\frac{\alpha_t}{\alpha}\left( \alpha
   %     (u(y_t(\theta),\theta)-r_0)+Q_t(x,a,\theta) \right)
   %     \label{eq:Qtup-2}
   % \end{align}
   % where $\alpha\in (0,\min\{L^{-1},1\})$ and we have suppressed the dependence
   % of $\alpha_t$ on $(x,a)$.
   % Let $\tilde{u}(y, \theta)=u(y,\theta)-r_0$. Then we define the map $T$ such
   % that
   % \begin{equation}
   %     (TQ_t)(x,a,\theta)=\alpha \mb{E}_{x,a}
   %     \tilde{u}(y_t(\theta),\theta)+Q_t(x,a, \theta)
   %     \label{eq:Tupdate}
   % \end{equation}
   % where $y_t(\theta)=r_t+\gamma \max_{a'\in
   % A}Q_t(x_{t+1},a,\theta)-Q_t(x_t,a,\theta)$. 
%\tc{red}{Add some comments on contravariant/natural gradients}

%The bulk of the argument for the proof of Theorem~\ref{thm:DQ} follows the
%structure of the proof
%of Proposition~4 in~\cite{neu:2007aa} with some modifications given the
%non-linear mapping of the temporal differences.

Let us briefly remark that the gradient algorithm and Theorem~\ref{thm:DQ} are
consistent with the gradient descent framework which uses the 
\emph{contravariant} gradient for learning as introduced in~\cite{amari:1998aa}
for Riemannian parameter spaces $\Theta$. Of course, when $\Theta$ is Euclidean
and the coordinate system is orthonormal, the gradient we normally use
(\emph{covariant} derivative) coincides with the contravariant gradient.
However, this suggests our techniques will not generalize to admissible parameter
spaces with more structure. 

Moreover, as is pointed out in~\cite{neu:2007aa},
the trajectories that result from the solution to the gradient algorithm are
equivalent up to reparameterization through a smooth invertible mapping with a
smooth inverse. Contravariant gradient methods have been shown to be
asymptotically efficient in a probabilistic sense and thus, they tend to avoid
\emph{plateaus}~\cite{amari:1998aa,peters:2005aa}.

Before we dive into the proof of Theorem~\ref{thm:DQ}, let us introduce some
definitions and useful propositions.

\begin{defn}[Fr{\'{e}}chet Subdifferentials] Let $U$ be a Banach space and $U^\ast$
    its dual. The Fr{\'{e}}chet subdifferential of $f: U\rar \mb{R}$ at $u\in
    U$, denoted by $\partial f(u)$ is the set of $u^\ast\in U^\ast$ such that
    \begin{equation}
        \lim_{h\rar 0}\inf_{h\neq 0} \|h\|^{-1}\left( f(u+h)-f(u)-\langle
        u^\ast, u\rangle \right)\geq 0
        \label{eq:def}
    \end{equation}
\end{defn}
%We require two propositions to complete the proof. 
\begin{prop}[\cite{neu:2007aa,kruger:2003aa}]
    For a finite family $(f_i)_{i\in I}$ of real-valued functions 
    (where $I$ is a finite index set) defined on $U$, let $f(u)=\max_{i\in I}
    f_i(u)$. If $u^\ast\in\partial f_i(u)$ and $f_i(u)=f(u)$, then $u^\ast\in
    \partial f_i(u)$. If $f_1,f_2: U\rar \mb{R}$, $\alpha_1,\alpha_2\geq 0$,
    then $\alpha_1\partial f_1+\alpha_2\partial f_2 \subset \partial
    (\alpha_1f_1+\alpha_1f_2)$.
    \label{prop:subdiff}
\end{prop}
\begin{prop}[\cite{neu:2007aa,penot:1995aa}]
    Suppose that $(f_n)_{n\in \mb{N}}$ is a sequence of real-valued functions on
    $U$ which converge pointwise to $f$. Let $u\in U$, $u_n^\ast\in \partial
    f_n(u)\subset U^\ast$ and suppose that $(u_n^\ast)$ is weak$^\ast$--convergent to
    $u^\ast$ and is bounded. Moreover, suppose that at $u$, for any $\vep>0$,
    there exists an $N>0$ and $\delta>0$ such that for any $n\geq N$, $h\in
    B_U(0,\delta)$, a $\delta$--ball around
    $0$, $f_n(u+h)\geq f_n(u)+\langle u_n^\ast,h\rangle -\vep \|h\|$. Then
    $u^\ast\in \partial f(u)$.
    \label{prop:subdiffconverge}
\end{prop}

We now provide the proof for parts (a) and (b) of Theorem~\ref{thm:DQ}.

\emph{proof of Theorem~\ref{thm:DQ}, part (a).}
    Let $Q_0(x,a,\theta)\equiv 0$. Then it is trivial that $Q_0(x,a,\theta)$ is
    locally Lipschitz in $\theta$ on $\Theta$. Supposing that $Q_t(x,a,\theta)$
    is $L_t$--locally Lipschitz in $\theta$, then we need to show that $TQ_t(x,a,\theta)$
    is locally Lipschitz which we recall is   defined by \begin{equation}
        (TQ)(x,a,\theta)=\alpha \mb{E}_{x,a,w}
        \tilde{
        \uv}(y(\theta),\theta)+Q(x,a, \theta)
        \label{eq:Tupdate}
    \end{equation}
    where $y(\theta)=r(x,a,w)+\gamma \max_{a'\in
    A}Q(x',a,\theta)-Q(x,a,\theta)$. 

   
    Since $\tilde{\uv}\equiv \uv-\uv_0$, it also satisfies Assumption~\ref{ass:u}. Let
    $L_y=\min\{L_y(\theta)| \theta\in \Theta\}$ and define
    $g(x,\theta)=\max_{a'}Q(x,a',\theta)$. Then, we have that
    %Thus, $\tilde{u}$ is monotonic in $x$ so that there exists a $\xi_{(x,y)}\in
    %[\epsilon,L]$ such that $\tilde{u}(x)-\tilde{u}(y)=\xi_{(x,y)}(x-y)$.
    \begin{align*}
       &\| TQ_t(\theta)-TQ_t(\theta')\|\notag\\
       &\quad\leq \alpha L_y\|
      y(\theta)-y(\theta')]\|+\alpha L_\theta\|\theta-\theta'\|+\|Q_t(\theta)-Q_t(\theta')\|\\
       &\quad\leq \alpha \gamma L_y \| g(s',\theta)-g(s',\theta')\|  +\alpha
       L_\theta\|\theta-\theta'\|\notag\\
       &\qquad+(1-\alpha \vep)\|Q_t(\theta)-Q_t(\theta')\|\\
        &\quad\leq (1-\alpha
       (1-\gamma)L_y)\|Q_t(\theta)-Q_t(\theta')\|+\alpha
       L_\theta \|\theta-\theta'\|\\
       &\quad\leq ((1-\alpha
       (1-\gamma)L_y)L_t+\alpha L_\theta)\|\theta-\theta'\|
    \end{align*}
%    \begin{align*}
%       \| TQ_t(\theta)-TQ_t(&\theta')\|\leq \alpha L_y\|
%      y(\theta)-y(\theta')]\|+\alpha L_\theta\|\theta-\theta'\|\\ % \mb{E}_{s,a}[\xi_{(x,x')}
%       &\qquad\qquad+\|Q_t(\theta)-Q_t(\theta')\|\\
%      % &\leq \alpha \gamma \|
%      % \mb{E}_{s,a}[\xi_{(x,x')}(\max_{a'}Q_i(s,a',\theta)-\max_{a'}Q_i(s,a',\theta')]\|\\
%       &\leq \alpha \gamma L_y \| v(s',\theta)-v(s',\theta')\|+\alpha
%       L_\theta \|\theta-\theta'\|\\
%%       \max_{a'}Q_i(s,a',\theta)-\max_{a'}Q_i(s,a',\theta')\|\\
%      % &+(1-\alpha\mb{E}_{s,a}[\xi_{(x,x')}])\|Q_i(\theta)-Q_i(\theta')\|+\alpha
%      % L_\theta \|\theta-\theta'\|\\
%        &\quad+(1-\alpha L_y)\|Q_t(\theta)-Q_t(\theta')\|\\
%      % &\leq (1-\alpha
%      % (1-\gamma)\mb{E}_{s,a}[\xi_{(x,x')}])\|Q_i(\theta)-Q_i(\theta')\|\\
%      % &+\alpha
%      % L_\theta \|\theta-\theta'\|\\
%        &\leq (1-\alpha
%       (1-\gamma)L_y)\|Q_t(\theta)-Q_t(\theta')\|\\
%       &\quad+\alpha
%       L_\theta \|\theta-\theta'\|\\
%       &\leq ((1-\alpha
%       (1-\gamma)L_y)L_t+\alpha L_\theta)\|\theta-\theta'\|
%    \end{align*}
    where we have suppressed the dependence of $Q_t(\cdot, \cdot, \theta)$ on
    $(x,a)$.
    Hence, letting $\bar{\alpha}=1-\alpha
    (1-\gamma)L_y$ we have that $TQ_t(\cdot, \cdot, \theta)$ is
    $L_{t+1}$--locally Lipschitz with $L_{t+1}=\bar{\alpha}L_t+\alpha L_\theta$.
    With $L_0=0$, by iterating we get that
       \begin{align*}
           L_{t+1}&=(\bar{\alpha}^{t}+\cdots +\bar{\alpha}+1)\alpha L_\theta
           %(\bar{\alpha}(\bar{\alpha}L_{i-1}+\alpha L_\theta))+\alpha L_\theta)\\
          % &=\bar{\alpha}^2L_{i-1}+\bar{\alpha}L_\theta+\alpha L_\theta\\
          % &=\bar{\alpha}^{i+1}L_0+L_\theta(\alpha+\bar{\alpha}+\cdots
          % +\bar{\alpha}^i)
       \end{align*}
       As stated in Section~\ref{sec:irlgrad}, $T$ is a contraction so that
       $T^nQ_0\rar Q^\ast_\theta=Q^\ast(\cdot, \cdot,
       \theta)$ as $n\rar\infty$.
       %Hence, $Q_\theta^\ast=Q^\ast(\cdot, \cdot,
       %\theta)=\lim_{n\rar\infty} T^nQ_0$. 
Hence, by the above argument $Q^\ast_\theta$ is $\alpha
L_\theta/(1-\bar{\alpha})$--Lipschitz continuous.
   \hfill\ensuremath{\blacksquare}

   \emph{proof of Theorem~\ref{thm:DQ}, part (b).}    Consider a fixed vector $\theta\in \mb{R}^d$.  We now show that the
      operator $S$ acting on the space of functions $\phi_\theta:X\times A\rar
      \mb{R}^d$ and 
      defined 
by
\begin{align}
           (S\phi_\theta)(x,a)
           =&\alpha \mb{E}_{x,a,w}\big[ D_\theta
           \tilde{\uv}(y(\theta),\theta)+D_y\tilde{\uv}(y(\theta), \theta)\notag\\
           &\quad\cdot(\gamma
       \phi_\theta(x',a_{x'}^\ast)-\phi_\theta(x,a)) \big]+\phi_\theta(x,a)
           \label{eq:Scontraction}
       \end{align}
              is a contraction where $a_{x'}^\ast$  is the action that maximizes $\sum_{a'\in
       A}\pi(a|x)Q(x,a,\theta)$.
              Indeed,
%\begin{align*}
%    (S\phi_\theta-&S\phi_\theta')(x,a)=\alpha
%    \mb{E}_{x,a,w}[
%D_y\tilde{u}(y(\theta),\theta)\big(\gamma  (\phi_\theta(x',a^\ast)\notag\\
%&\quad-\phi_\theta'(x',a^\ast))
%    -(\phi_\theta(x,a)-\phi_\theta'(x,a))\big)]\notag\\
%    &\qquad+\phi_\theta(x,a)-\phi_\theta'(x,a)\\
%    &\leq \alpha\gamma
%    \mb{E}_{x,a,w}[D_y\tilde{u}(y(\theta),\theta)(\phi_\theta(x',a^\ast_{x'})-\phi_\theta'(x',a^\ast_{x'}))]\\
%    &+(1-\alpha
%    \mb{E}_{x,a,w}[D_y\tilde{u}(y(\theta),\theta)])(\phi_\theta(x,a)-\phi_\theta'(x,a))
%  %  &\leq (1-\alpha(1-\gamma)L_y)\|\phi-\phi'\|_\infty
%\end{align*}
\begin{align*}
    &(S\phi_\theta-S\phi_\theta')(x,a)\notag\\
    &=\alpha
    \mb{E}_{x,a,w}[
D_y\tilde{\uv}(y(\theta),\theta)\big(\gamma  (\phi_\theta(x',a^\ast)-\phi_\theta'(x',a^\ast))
    -(\phi_\theta(x,a)\notag\\
&\qquad-\phi_\theta'(x,a))\big)]+\phi_\theta(x,a)-\phi_\theta'(x,a)\\
    &\leq \alpha\gamma
    \mb{E}_{x,a,w}[D_y\tilde{\uv}(y(\theta),\theta)(\phi_\theta(x',a^\ast_{x'})-\phi_\theta'(x',a^\ast_{x'}))]\\
    &\qquad+(1-\alpha
    \mb{E}_{x,a,w}[D_y\tilde{\uv}(y(\theta),\theta)])(\phi_\theta(x,a)-\phi_\theta'(x,a))
  %  &\leq (1-\alpha(1-\gamma)L_y)\|\phi-\phi'\|_\infty
\end{align*}
so that
%\begin{align*}
$\|(S\phi_\theta- S\phi_\theta')(x,a)\|\leq
(1-\alpha(1-\gamma)L_y)\|\phi_\theta-\phi_\theta'\|_\infty$
%\end{align*}
since for a differentiable Lipschitz map the norm of the derivative is always
bounded above by the Lipschitz constant.
%inequality {\displaystyle \|Df\|_{\infty ,U}\leq K} \|Df\|_{\infty ,U}\leq K holds for the best Lipschitz constant of f,
Thus, $\bar{\alpha}$ is the required constant for ensuring $S$ is a contraction.
We remark that $S$ operates on each of the $d$ components of $\theta$ separately
and hence, it is a contraction when restricted to each individual component.

Let $\pi$ denote a greedy policy with respect to $Q^\ast_\theta$ and let $\pi_n$
be a sequence of policies that are greedy with respect to $Q_n=T^nQ_0$ where
ties are broken so that $\sum_{(x,a)\in X\times A}|\pi(a|x)-\pi_n(a|x)|$ is
minimized. Then for large enough $n$, $\pi_n=\pi$. Denote by $S_{\pi_n}$ the map
$S$ defined in \eqref{eq:Scontraction} where $\pi_n$ is the implemented policy. Consider the sequence
$\phi_{\theta,n}$ such that $\phi_{\theta,0}=0$ and
$\phi_{\theta,n+1}=S_{\pi_n}\phi_{\theta,n}$. For large enough $n$,
$\phi_{\theta, n+1}=S_{\pi}\phi_{\theta,n}$. 
%Hence, $\phi_{\theta,n}\in  D_\theta Q_n$ holds for $n\geq 0$ by induction.
%Note that $\phi_{\theta,0       
Applying the (local) contraction mapping theorem (see,
\emph{e.g.},~\cite[Theorem~3.18]{sastry:1999aa}) we get that
$\lim_{n\rar\infty} S^n\phi_0$
converges to a unique fixed point.
Moreover, by induction and Proposition~\ref{prop:subdiff}, $\phi_{\theta,n}(x,a)\in
\partial_\theta Q_n(x,a,\theta)$. Hence, by
Proposition~\ref{prop:subdiffconverge}, the limit is a subdifferential of
$Q_\theta^\ast$ since $\tilde{\uv}$ is Lipschitz on $Y$ and $\theta$ and the
derivatives of $\tilde{\uv}$ are uniformly bounded.
Since by part (a) $Q^\ast_\theta$ is locally Lipschitz in $\theta$, Rademacher's
Theorem (see, \emph{e.g.},~\cite[Thm.~3.1]{heinonen:2004aa}) tells us it is differentiable almost everywhere (expcept a set of Lebesgue measure zero). Since $Q_\theta^\ast$ is
differentiable, its subdifferential is its derivative.
\hfill\ensuremath{\blacksquare}

      % Let $\pi$ denote a greedy policy with respect to $Q_\theta^\ast$ and let
      % $\pi_n$ be a sequenece of policies that are greedy with respect to $Q_n$
      % (with ties broken so that $\sum_{(s,a)\in S\times
      % A}|\pi(a|s)-\pi_n(a|s)|$ is minimized). 
       %where $S$ operates on $D_\theta Q$:
       %    By
%    adding and subtracting $\tilde{u}(x_t(\theta),\theta')$ we have
%    that
%    \begin{align*}
%        \|\tilde{u}(x_t(\theta),\theta)-\tilde{u}(x_t(\theta'),\theta')\|&\leq
%        \|\tilde{u}(x_t(\theta),\theta)+\tilde{u}(x_t(\theta),\theta')\|\notag\\
%        %=\|\tilde{u}(x_t(\theta),\theta)+\tilde{u}(x_t(\theta),\theta')\notag\\
%       %&\qquad\qquad\qquad\qquad\qquad -\tilde{u}(x_t(\theta),\theta')-\tilde{u}(x_t(\theta'),\theta')\|\\
%        &+\|\tilde{u}(x_t(\theta),\theta')-\tilde{u}(x_t(\theta'),\theta')\|\\
%        &\leq L_\theta\|\theta-\theta'\|\\
%        &+ L_x\|x_t(\theta)-x_t(\theta)'\|\\
%        &\leq (L_\theta+R(\gamma+1)L_x)\|\theta-\theta'\|
%    %    \label{eq:kk}
%    \end{align*}
%Let $L_u= L_\theta+R(\gamma+1)L_x$. Now let us see a few iterations:
%\begin{align*}
%    &\|TQ_0(\theta_1)-TQ_0(\theta_2)\|\leq
%    \alpha\|\tilde{u}(x(Q_0(\theta_1)),\theta_1)-
%    \tilde{u}(x(Q_0(\theta_2)),\theta_2)\|\\
%    &+\|Q_0(\theta_1)-Q_0(\theta_2)\|\\
%&\leq \alpha L_\theta\|\theta_1-\theta_2\|+R\|\theta_1-\theta_2\|+\alpha L_x\|x(Q_0(\theta_1))-x(Q_0(\theta_2))\|\\
%&\leq (\alpha L_\theta+R)\|\theta_1-\theta_2\|+\alpha L_x(1+\gamma)R\|\theta_1-\theta_2\|
%\end{align*}
%so that
%\begin{equation*}
%    \|TQ_0(\theta_1)-TQ_0(\theta_2)\|=\|Q_1(\theta_1)-Q_1(\theta_2)\|\leq L_1\|\theta_1-\theta_2\|
%\end{equation*}
%where $L_1=(\alpha L_u+R)$.
%Now consider the next iteration:
%\begin{align*}
%    &\|TQ_1(\theta_1)-TQ_1(\theta_2)\|\leq
%    \alpha\|\tilde{u}(x(Q_1(\theta_1)),\theta_1)-
%    \tilde{u}(x(Q_1(\theta_2)),\theta_2)\|\\
%    &+\|Q_1(\theta_1)-Q_1(\theta_2)\|\\
%&\leq \alpha L_\theta\|\theta_1-\theta_2\|+L_1\|\theta_1-\theta_2\|+\alpha
%L_x\|x(Q_1(\theta_1))-x(Q_1(\theta_2))\|\\
%&\leq (\alpha L_\theta+L_1)\|\theta_1-\theta_2\|+\alpha
%L_x(1+\gamma)L_1\|\theta_1-\theta_2\|\\
%&= (\alpha L_\theta +L_1(1+\alpha L_x(1+\gamma)))\|\theta_1-\theta_2\|\\
%&=(\alpha L_\theta + (\alpha L_u+R)(1+\alpha L_x(1+\gamma)))\|\theta_1-\theta_2\|
%\end{align*}
%Expanding we get the following constant which we define to be $L_2$:
%\[L_2=R+2\alpha L_u+\alpha^2 L_u L_x(1+\gamma)\]
%so that
%\[\|Q_2(\theta_1)-Q_2(\theta_2)\|\leq L_2\|\theta_1-\theta_2\|\]
%Let's do one more iteration:
%\begin{align*}
%    &\|TQ_2(\theta_1)-TQ_2(\theta_2)\|\leq
%    \alpha\|\tilde{u}(x(Q_2(\theta_1)),\theta_1)-
%    \tilde{u}(x(Q_2(\theta_2)),\theta_2)\|\\
%    &+\|Q_2(\theta_1)-Q_2(\theta_2)\|\\
%&\leq \alpha L_\theta\|\theta_1-\theta_2\|+L_2\|\theta_1-\theta_2\|+\alpha
%L_x\|x(Q_2(\theta_1))-x(Q_2(\theta_2))\|\\
%&\leq (\alpha L_\theta+L_2)\|\theta_1-\theta_2\|+\alpha
%L_x(1+\gamma)L_2\|\theta_1-\theta_2\|\\
%%&= (\alpha L_\theta +L_1(1+\alpha L_x(1+\gamma)))\|\theta_1-\theta_2\|\\
%%&=(\alpha L_\theta + (\alpha L_u+R)(1+\alpha L_x(1+\gamma)))\|\theta_1-\theta_2\|
%\end{align*}
%Plugging in $L_2$ and doing some algebra, we get that the constant is
%\[L_3=\alpha^3L_u(L_x(1+\gamma))^2+3\alpha^2L_x(1+\gamma)L_u+ 3\alpha L_u+R\]
%Continuing in this fashion we can derive that
%\begin{align*}
%    L_4=&\alpha^4L_u(L_x(1+\gamma))^3+4\alpha^3L_u(L_x(1+\gamma))^2\\
%    &+4L_u\alpha^2L_x(1+\gamma)L_u+4\alpha
%    L_u+R\end{align*}
%and so on so that
%\begin{align*}
%    L_k=R+\alpha^kL_u(L_x(1+\gamma))^{k-1}+kL_u\sum_{i=1}^{k-1}
%    \alpha^i(L_x(1+\gamma))^{i-1}
%\end{align*}
%\end{proof}




==> proofThmQ_oldv1.tex <==

%\begin{proof}
   % Let $L=\max_\theta\{L_y(\theta),L_\theta\}$. We re-write our $Q$--update equation as follows:
   % \begin{align}
   %     Q_{t+1}(x,a,\theta)=&\left( 1-\frac{\alpha_t}{\alpha}
   %     \right)Q_t(x,a,\theta)\notag\\
   %     &\quad+\frac{\alpha_t}{\alpha}\left( \alpha
   %     (u(y_t(\theta),\theta)-r_0)+Q_t(x,a,\theta) \right)
   %     \label{eq:Qtup-2}
   % \end{align}
   % where $\alpha\in (0,\min\{L^{-1},1\})$ and we have suppressed the dependence
   % of $\alpha_t$ on $(x,a)$.
   % Let $\tilde{u}(y, \theta)=u(y,\theta)-r_0$. Then we define the map $T$ such
   % that
   % \begin{equation}
   %     (TQ_t)(x,a,\theta)=\alpha \mb{E}_{x,a}
   %     \tilde{u}(y_t(\theta),\theta)+Q_t(x,a, \theta)
   %     \label{eq:Tupdate}
   % \end{equation}
   % where $y_t(\theta)=r_t+\gamma \max_{a'\in
   % A}Q_t(x_{t+1},a,\theta)-Q_t(x_t,a,\theta)$. 
%\tc{red}{Add some comments on contravariant/natural gradients}

%The bulk of the argument for the proof of Theorem~\ref{thm:DQ} follows the
%structure of the proof
%of Proposition~4 in~\cite{neu:2007aa} with some modifications given the
%non-linear mapping of the temporal differences.

Let us briefly remark that the gradient algorithm and Theorem~\ref{thm:DQ} are
consistent with the gradient descent framework which uses the 
\emph{contravariant} gradient for learning as introduced in~\cite{amari:1998aa}
for Riemannian parameter spaces $\Theta$. Of course, when $\Theta$ is Euclidean
and the coordinate system is orthonormal, the gradient we normally use
(\emph{covariant} derivative) coincides with the contravariant gradient.
However, this suggests our techniques will not generalize to admissible parameter
spaces with more structure. 

Moreover, as is pointed out in~\cite{neu:2007aa},
the trajectories that result from the solution to the gradient algorithm are
equivalent up to reparameterization through a smooth invertible mapping with a
smooth inverse. Contravariant gradient methods have been shown to be
asymptotically efficient in a probabilistic sense and thus, they tend to avoid
\emph{plateaus}~\cite{amari:1998aa,peters:2005aa}.

Before we dive into the proof of Theorem~\ref{thm:DQ}, let us introduce some
definitions and useful propositions.

\begin{defn}[Fr{\'{e}}chet Subdifferentials] Let $U$ be a Banach space and $U^\ast$
    its dual. The Fr{\'{e}}chet subdifferential of $f: U\rar \mb{R}$ at $u\in
    U$, denoted by $\partial f(u)$ is the set of $u^\ast\in U^\ast$ such that
    \begin{equation}
        \lim_{h\rar 0}\inf_{h\neq 0} \|h\|^{-1}\left( f(u+h)-f(u)-\langle
        u^\ast, u\rangle \right)\geq 0
        \label{eq:def}
    \end{equation}
\end{defn}
%We require two propositions to complete the proof. 
\begin{prop}[\cite{neu:2007aa,kruger:2003aa}]
    For a finite family $(f_i)_{i\in I}$ of real-valued functions 
    (where $I$ is a finite index set) defined on $U$, let $f(u)=\max_{i\in I}
    f_i(u)$. If $u^\ast\in\partial f_i(u)$ and $f_i(u)=f(u)$, then $u^\ast\in
    \partial f_i(u)$. If $f_1,f_2: U\rar \mb{R}$, $\alpha_1,\alpha_2\geq 0$,
    then $\alpha_1\partial f_1+\alpha_2\partial f_2 \subset \partial
    (\alpha_1f_1+\alpha_1f_2)$.
    \label{prop:subdiff}
\end{prop}
\begin{prop}[\cite{neu:2007aa,penot:1995aa}]
    Suppose that $(f_n)_{n\in \mb{N}}$ is a sequence of real-valued functions on
    $U$ which converge pointwise to $f$. Let $u\in U$, $u_n^\ast\in \partial
    f_n(u)\subset U^\ast$ and suppose that $(u_n^\ast)$ is weak$^\ast$--convergent to
    $u^\ast$ and is bounded. Moreover, suppose that at $u$, for any $\vep>0$,
    there exists an $N>0$ and $\delta>0$ such that for any $n\geq N$, $h\in
    B_U(0,\delta)$, a $\delta$--ball around
    $0$, $f_n(u+h)\geq f_n(u)+\langle u_n^\ast,h\rangle -\vep \|h\|$. Then
    $u^\ast\in \partial f(u)$.
    \label{prop:subdiffconverge}
\end{prop}

We now provide the proof for parts (a) and (b) of Theorem~\ref{thm:DQ}.

\emph{proof of Theorem~\ref{thm:DQ}, part (a).}
    Let $Q_0(x,a,\theta)\equiv 0$. Then it is trivial that $Q_0(x,a,\theta)$ is
    locally Lipschitz in $\theta$ on $\Theta$. Supposing that $Q_t(x,a,\theta)$
    is $L_t$--locally Lipschitz in $\theta$, then we need to show that $TQ_t(x,a,\theta)$
    is locally Lipschitz which we recall is   defined by \begin{equation}
        (TQ)(x,a,\theta)=\alpha \mb{E}_{x',w}
        \tilde{
        \uv}(y(\theta),\theta)+Q(x,a, \theta)
        \label{eq:Tupdate}
    \end{equation}
    where $y(\theta)=r(x,a,w)+\gamma \max_{a'\in
    A}Q(x',a',\theta)-Q(x,a,\theta)$. 

   
    Since $\tilde{\uv}\equiv \uv-\uv_0$, it also satisfies Assumption~\ref{ass:u}. Let
    $L_y=\max\{L_y(\theta)| \theta\in \Theta\}$ and define
    $g_t(x,\theta)=\max_{a'}Q_t(x,a',\theta)$. Note that since $Q_t$ is assumed
    Lipschitz with constant $L_t$, so is $g_t$. is Then, we have that
    %Thus, $\tilde{u}$ is monotonic in $x$ so that there exists a $\xi_{(x,y)}\in
    %[\epsilon,L]$ such that $\tilde{u}(x)-\tilde{u}(y)=\xi_{(x,y)}(x-y)$.
    \begin{align*}
        TQ_t(\theta)-TQ_t(\theta')&=\alpha \mb{E}_{x',w}[\tilde{
        \uv}(y(\theta),\theta)-\tilde{
        \uv}(y(\theta'),\theta')]\\
        &\ \ +Q_t(x,a,\theta)-Q_t(x,a,\theta')\\
        &=\alpha\mb{E}_{x',w}[\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta)\\
            &\ \ +\tilde{v}(y(\theta'),\theta)-\tilde{
        \uv}(y(\theta'),\theta')]\\
        &\ \ +Q_t(\theta)-Q_t(\theta')
    \end{align*}
    where we have surpressed the dependence on $(x,a)$.
    Now, due to the monotonicity of $\tilde{v}$ in $y$, we know that for all
    $y_1,y_2$ there exists $\xi\in[\vep,L_y]$ such that
    \[\tilde{v}(y_1,\theta)-\tilde{v}(y_2,\theta)=\xi(y_1-y_2)\]
    Hence, 
\begin{align*}
    &    \mb{E}_{x',w}[\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta)+\tilde{v}(y(\theta'),\theta)-\tilde{
        \uv}(y(\theta'),\theta')]\\
        &\ \ = \mb{E}_{x',w}[\xi_{x',w}(y(\theta)-y(\theta'))+\tilde{v}(y(\theta'),\theta)-\tilde{
        \uv}(y(\theta'),\theta')]
    \end{align*}
    where we simply denote the dependence of $\xi$ on the $x'$ and $w$.
    %since
    %\[
Then,
    \begin{align*}
       & TQ_t(\theta)-TQ_t(\theta')\\
       &\ \ =\alpha\mb{E}_{x',w}[\xi_{x',w}(y(\theta)-y(\theta')) +\tilde{v}(y(\theta'),\theta)-\tilde{
        \uv}(y(\theta'),\theta')]\\
        &\qquad +Q_t(\theta)-Q_t(\theta')\\
        %%
        &\ \ =\alpha\gamma\mb{E}_{x',w}[\xi_{x',w}(g_t(x',\theta)-g_t(x',\theta'))]-\alpha\mb{E}_{x',w}[\xi_{x',w}(Q_t(\theta)
    \\
&\qquad-Q_t(\theta'))]+\alpha \mb{E}_{x',w}[\tilde{v}(y(\theta'),\theta)-\tilde{
        \uv}(y(\theta'),\theta')]\\
        &\qquad +Q_t(\theta)-Q_t(\theta')\\
        %%
        &\ \
        =\alpha\gamma\mb{E}_{x',w}[\xi_{x',w}(g_t(x',\theta)-g_t(x',\theta'))]-\alpha\mb{E}_{x',w}[\xi_{x',w}](Q_t(\theta)
\\
    &\qquad    -Q_t(\theta'))]+\alpha \mb{E}_{x',w}[\tilde{v}(y(\theta'),\theta)-\tilde{
        \uv}(y(\theta'),\theta')]\\
        &\qquad +Q_t(\theta)-Q_t(\theta')\\
        %%
        &\ \ =(1-\alpha\mb{E}_{x',w}[\xi_{x',w}])(Q_t(\theta)
    -Q_t(\theta'))+\alpha\gamma\mb{E}_{x',w}[\xi_{x',w}\\
    &\qquad\cdot (g_t(x',\theta)-g_t(x',\theta'))] +\alpha \mb{E}_{x',w}[\tilde{v}(y(\theta'),\theta)-\tilde{
        \uv}(y(\theta'),\theta')]
    \end{align*}
 %   Letting $\tilde{P}(x',w|x,a)=P(x'|a,x)P_r(w|x,a)$, we have
    %% Indeed, 
    % \[||\mb{E}_{x',w}[\tilde{v}(y(\theta'),\theta)-\tilde{
%\uv}(y(\theta'),\theta')]||\leq\sum_{x',w}
%\tilde{P}(x',w)||\tilde{v}-\tilde{v}'\|\]
% and $\sum \tilde{P}=1$.
    so that
    \begin{align*}
      &\| TQ_t(\theta)-TQ_t(\theta')\| \leq (((1-\alpha(1-\gamma) \vep))+\alpha L_\theta)L_t\|\theta-\theta'\|
      %\|Q_t(\theta)-Q_t(\theta')\|+\alpha\gamma
      %L_y\|g_t(x',\theta)-g_t(x',\theta')\|
  \end{align*}
 %  
 %   \begin{align*}
 %      &\| TQ_t(\theta)-TQ_t(\theta')\|\notag\\
 %      &\quad\leq \alpha L_y\|
 %     y(\theta)-y(\theta')]\|+\alpha L_\theta\|\theta-\theta'\|+\|Q_t(\theta)-Q_t(\theta')\|\\
 %      &\quad\leq \alpha \gamma L_y \| g(s',\theta)-g(s',\theta')\|  +\alpha
 %      L_\theta\|\theta-\theta'\|\notag\\
 %      &\qquad+(1-\alpha \vep)\|Q_t(\theta)-Q_t(\theta')\|\\
 %       &\quad\leq (1-\alpha
 %      (1-\gamma)L_y)\|Q_t(\theta)-Q_t(\theta')\|+\alpha
 %      L_\theta \|\theta-\theta'\|\\
 %      &\quad\leq ((1-\alpha
 %      (1-\gamma)L_y)L_t+\alpha L_\theta)\|\theta-\theta'\|
 %   \end{align*}
 %   \begin{align*}
 %      \| TQ_t(\theta)-TQ_t(&\theta')\|\leq \alpha L_y\|
 %     y(\theta)-y(\theta')]\|+\alpha L_\theta\|\theta-\theta'\|\\ % \mb{E}_{s,a}[\xi_{(x,x')}
 %      &\qquad\qquad+\|Q_t(\theta)-Q_t(\theta')\|\\
 %     % &\leq \alpha \gamma \|
 %     % \mb{E}_{s,a}[\xi_{(x,x')}(\max_{a'}Q_i(s,a',\theta)-\max_{a'}Q_i(s,a',\theta')]\|\\
 %      &\leq \alpha \gamma L_y \| v(s',\theta)-v(s',\theta')\|+\alpha
 %      L_\theta \|\theta-\theta'\|\\
%%       \max_{a'}Q_i(s,a',\theta)-\max_{a'}Q_i(s,a',\theta')\|\\
 %     % &+(1-\alpha\mb{E}_{s,a}[\xi_{(x,x')}])\|Q_i(\theta)-Q_i(\theta')\|+\alpha
 %     % L_\theta \|\theta-\theta'\|\\
 %       &\quad+(1-\alpha L_y)\|Q_t(\theta)-Q_t(\theta')\|\\
 %     % &\leq (1-\alpha
 %     % (1-\gamma)\mb{E}_{s,a}[\xi_{(x,x')}])\|Q_i(\theta)-Q_i(\theta')\|\\
 %     % &+\alpha
 %     % L_\theta \|\theta-\theta'\|\\
 %       &\leq (1-\alpha
 %      (1-\gamma)L_y)\|Q_t(\theta)-Q_t(\theta')\|\\
 %      &\quad+\alpha
 %      L_\theta \|\theta-\theta'\|\\
 %      &\leq ((1-\alpha
 %      (1-\gamma)L_y)L_t+\alpha L_\theta)\|\theta-\theta'\|
 %   \end{align*}
 %   where we have suppressed the dependence of $Q_t(\cdot, \cdot, \theta)$ on
 %   $(x,a)$.
    Hence, letting $\bar{\alpha}=1-\alpha
    (1-\gamma)\vep$ we have that $TQ_t(\cdot, \cdot, \theta)$ is
    $L_{t+1}$--locally Lipschitz with $L_{t+1}=\bar{\alpha}L_t+\alpha L_\theta$.
    With $L_0=0$, by iterating we get that
       \begin{align*}
           L_{t+1}&=(\bar{\alpha}^{t}+\cdots +\bar{\alpha}+1)\alpha L_\theta
           %(\bar{\alpha}(\bar{\alpha}L_{i-1}+\alpha L_\theta))+\alpha L_\theta)\\
          % &=\bar{\alpha}^2L_{i-1}+\bar{\alpha}L_\theta+\alpha L_\theta\\
          % &=\bar{\alpha}^{i+1}L_0+L_\theta(\alpha+\bar{\alpha}+\cdots
          % +\bar{\alpha}^i)
       \end{align*}
       As stated in Section~\ref{sec:irlgrad}, $T$ is a contraction so that
       $T^nQ_0\rar Q^\ast_\theta=Q^\ast(\cdot, \cdot,
       \theta)$ as $n\rar\infty$.
       %Hence, $Q_\theta^\ast=Q^\ast(\cdot, \cdot,
       %\theta)=\lim_{n\rar\infty} T^nQ_0$. 
Hence, by the above argument $Q^\ast_\theta$ is $\alpha
L_\theta/(1-\bar{\alpha})$--Lipschitz continuous.
   \hfill\ensuremath{\blacksquare}

   \emph{proof of Theorem~\ref{thm:DQ}, part (b).}    Consider a fixed vector $\theta\in \mb{R}^d$.  We now show that the
      operator $S$ acting on the space of functions $\phi_\theta:X\times A\rar
      \mb{R}^d$ and 
      defined 
by
\begin{align}
           (S\phi_\theta)(x,a)
           =&\alpha \mb{E}_{x,a,w}\big[ D_\theta
           \tilde{\uv}(y(\theta),\theta)+D_y\tilde{\uv}(y(\theta), \theta)\notag\\
           &\quad\cdot(\gamma
       \phi_\theta(x',a_{x'}^\ast)-\phi_\theta(x,a)) \big]+\phi_\theta(x,a)
           \label{eq:Scontraction}
       \end{align}
              is a contraction where $a_{x'}^\ast$  is the action that maximizes $\sum_{a'\in
       A}\pi(a|x)Q(x,a,\theta)$.
              Indeed,
%\begin{align*}
%    (S\phi_\theta-&S\phi_\theta')(x,a)=\alpha
%    \mb{E}_{x,a,w}[
%D_y\tilde{u}(y(\theta),\theta)\big(\gamma  (\phi_\theta(x',a^\ast)\notag\\
%&\quad-\phi_\theta'(x',a^\ast))
%    -(\phi_\theta(x,a)-\phi_\theta'(x,a))\big)]\notag\\
%    &\qquad+\phi_\theta(x,a)-\phi_\theta'(x,a)\\
%    &\leq \alpha\gamma
%    \mb{E}_{x,a,w}[D_y\tilde{u}(y(\theta),\theta)(\phi_\theta(x',a^\ast_{x'})-\phi_\theta'(x',a^\ast_{x'}))]\\
%    &+(1-\alpha
%    \mb{E}_{x,a,w}[D_y\tilde{u}(y(\theta),\theta)])(\phi_\theta(x,a)-\phi_\theta'(x,a))
%  %  &\leq (1-\alpha(1-\gamma)L_y)\|\phi-\phi'\|_\infty
%\end{align*}
\begin{align*}
    &(S\phi_\theta-S\phi_\theta')(x,a)\notag\\
    &=\alpha
    \mb{E}_{x,a,w}[
D_y\tilde{\uv}(y(\theta),\theta)\big(\gamma  (\phi_\theta(x',a^\ast)-\phi_\theta'(x',a^\ast))
    -(\phi_\theta(x,a)\notag\\
&\qquad-\phi_\theta'(x,a))\big)]+\phi_\theta(x,a)-\phi_\theta'(x,a)\\
    &\leq \alpha\gamma
    \mb{E}_{x,a,w}[D_y\tilde{\uv}(y(\theta),\theta)(\phi_\theta(x',a^\ast_{x'})-\phi_\theta'(x',a^\ast_{x'}))]\\
    &\qquad+(1-\alpha
    \mb{E}_{x,a,w}[D_y\tilde{\uv}(y(\theta),\theta)])(\phi_\theta(x,a)-\phi_\theta'(x,a))
  %  &\leq (1-\alpha(1-\gamma)L_y)\|\phi-\phi'\|_\infty
\end{align*}
so that
%\begin{align*}
$\|(S\phi_\theta- S\phi_\theta')(x,a)\|\leq
(1-\alpha(1-\gamma)L_y)\|\phi_\theta-\phi_\theta'\|_\infty$
%\end{align*}
since for a differentiable Lipschitz map the norm of the derivative is always
bounded above by the Lipschitz constant.
%inequality {\displaystyle \|Df\|_{\infty ,U}\leq K} \|Df\|_{\infty ,U}\leq K holds for the best Lipschitz constant of f,
Thus, $\bar{\alpha}$ is the required constant for ensuring $S$ is a contraction.
We remark that $S$ operates on each of the $d$ components of $\theta$ separately
and hence, it is a contraction when restricted to each individual component.

Let $\pi$ denote a greedy policy with respect to $Q^\ast_\theta$ and let $\pi_n$
be a sequence of policies that are greedy with respect to $Q_n=T^nQ_0$ where
ties are broken so that $\sum_{(x,a)\in X\times A}|\pi(a|x)-\pi_n(a|x)|$ is
minimized. Then for large enough $n$, $\pi_n=\pi$. Denote by $S_{\pi_n}$ the map
$S$ defined in \eqref{eq:Scontraction} where $\pi_n$ is the implemented policy. Consider the sequence
$\phi_{\theta,n}$ such that $\phi_{\theta,0}=0$ and
$\phi_{\theta,n+1}=S_{\pi_n}\phi_{\theta,n}$. For large enough $n$,
$\phi_{\theta, n+1}=S_{\pi}\phi_{\theta,n}$. 
%Hence, $\phi_{\theta,n}\in  D_\theta Q_n$ holds for $n\geq 0$ by induction.
%Note that $\phi_{\theta,0       
Applying the (local) contraction mapping theorem (see,
\emph{e.g.},~\cite[Theorem~3.18]{sastry:1999aa}) we get that
$\lim_{n\rar\infty} S^n\phi_0$
converges to a unique fixed point.
Moreover, by induction and Proposition~\ref{prop:subdiff}, $\phi_{\theta,n}(x,a)\in
\partial_\theta Q_n(x,a,\theta)$. Hence, by
Proposition~\ref{prop:subdiffconverge}, the limit is a subdifferential of
$Q_\theta^\ast$ since $\tilde{\uv}$ is Lipschitz on $Y$ and $\theta$ and the
derivatives of $\tilde{\uv}$ are uniformly bounded.
Since by part (a) $Q^\ast_\theta$ is locally Lipschitz in $\theta$, Rademacher's
Theorem (see, \emph{e.g.},~\cite[Thm.~3.1]{heinonen:2004aa}) tells us it is differentiable almost everywhere (expcept a set of Lebesgue measure zero). Since $Q_\theta^\ast$ is
differentiable, its subdifferential is its derivative.
\hfill\ensuremath{\blacksquare}

      % Let $\pi$ denote a greedy policy with respect to $Q_\theta^\ast$ and let
      % $\pi_n$ be a sequenece of policies that are greedy with respect to $Q_n$
      % (with ties broken so that $\sum_{(s,a)\in S\times
      % A}|\pi(a|s)-\pi_n(a|s)|$ is minimized). 
       %where $S$ operates on $D_\theta Q$:
       %    By
%    adding and subtracting $\tilde{u}(x_t(\theta),\theta')$ we have
%    that
%    \begin{align*}
%        \|\tilde{u}(x_t(\theta),\theta)-\tilde{u}(x_t(\theta'),\theta')\|&\leq
%        \|\tilde{u}(x_t(\theta),\theta)+\tilde{u}(x_t(\theta),\theta')\|\notag\\
%        %=\|\tilde{u}(x_t(\theta),\theta)+\tilde{u}(x_t(\theta),\theta')\notag\\
%       %&\qquad\qquad\qquad\qquad\qquad -\tilde{u}(x_t(\theta),\theta')-\tilde{u}(x_t(\theta'),\theta')\|\\
%        &+\|\tilde{u}(x_t(\theta),\theta')-\tilde{u}(x_t(\theta'),\theta')\|\\
%        &\leq L_\theta\|\theta-\theta'\|\\
%        &+ L_x\|x_t(\theta)-x_t(\theta)'\|\\
%        &\leq (L_\theta+R(\gamma+1)L_x)\|\theta-\theta'\|
%    %    \label{eq:kk}
%    \end{align*}
%Let $L_u= L_\theta+R(\gamma+1)L_x$. Now let us see a few iterations:
%\begin{align*}
%    &\|TQ_0(\theta_1)-TQ_0(\theta_2)\|\leq
%    \alpha\|\tilde{u}(x(Q_0(\theta_1)),\theta_1)-
%    \tilde{u}(x(Q_0(\theta_2)),\theta_2)\|\\
%    &+\|Q_0(\theta_1)-Q_0(\theta_2)\|\\
%&\leq \alpha L_\theta\|\theta_1-\theta_2\|+R\|\theta_1-\theta_2\|+\alpha L_x\|x(Q_0(\theta_1))-x(Q_0(\theta_2))\|\\
%&\leq (\alpha L_\theta+R)\|\theta_1-\theta_2\|+\alpha L_x(1+\gamma)R\|\theta_1-\theta_2\|
%\end{align*}
%so that
%\begin{equation*}
%    \|TQ_0(\theta_1)-TQ_0(\theta_2)\|=\|Q_1(\theta_1)-Q_1(\theta_2)\|\leq L_1\|\theta_1-\theta_2\|
%\end{equation*}
%where $L_1=(\alpha L_u+R)$.
%Now consider the next iteration:
%\begin{align*}
%    &\|TQ_1(\theta_1)-TQ_1(\theta_2)\|\leq
%    \alpha\|\tilde{u}(x(Q_1(\theta_1)),\theta_1)-
%    \tilde{u}(x(Q_1(\theta_2)),\theta_2)\|\\
%    &+\|Q_1(\theta_1)-Q_1(\theta_2)\|\\
%&\leq \alpha L_\theta\|\theta_1-\theta_2\|+L_1\|\theta_1-\theta_2\|+\alpha
%L_x\|x(Q_1(\theta_1))-x(Q_1(\theta_2))\|\\
%&\leq (\alpha L_\theta+L_1)\|\theta_1-\theta_2\|+\alpha
%L_x(1+\gamma)L_1\|\theta_1-\theta_2\|\\
%&= (\alpha L_\theta +L_1(1+\alpha L_x(1+\gamma)))\|\theta_1-\theta_2\|\\
%&=(\alpha L_\theta + (\alpha L_u+R)(1+\alpha L_x(1+\gamma)))\|\theta_1-\theta_2\|
%\end{align*}
%Expanding we get the following constant which we define to be $L_2$:
%\[L_2=R+2\alpha L_u+\alpha^2 L_u L_x(1+\gamma)\]
%so that
%\[\|Q_2(\theta_1)-Q_2(\theta_2)\|\leq L_2\|\theta_1-\theta_2\|\]
%Let's do one more iteration:
%\begin{align*}
%    &\|TQ_2(\theta_1)-TQ_2(\theta_2)\|\leq
%    \alpha\|\tilde{u}(x(Q_2(\theta_1)),\theta_1)-
%    \tilde{u}(x(Q_2(\theta_2)),\theta_2)\|\\
%    &+\|Q_2(\theta_1)-Q_2(\theta_2)\|\\
%&\leq \alpha L_\theta\|\theta_1-\theta_2\|+L_2\|\theta_1-\theta_2\|+\alpha
%L_x\|x(Q_2(\theta_1))-x(Q_2(\theta_2))\|\\
%&\leq (\alpha L_\theta+L_2)\|\theta_1-\theta_2\|+\alpha
%L_x(1+\gamma)L_2\|\theta_1-\theta_2\|\\
%%&= (\alpha L_\theta +L_1(1+\alpha L_x(1+\gamma)))\|\theta_1-\theta_2\|\\
%%&=(\alpha L_\theta + (\alpha L_u+R)(1+\alpha L_x(1+\gamma)))\|\theta_1-\theta_2\|
%\end{align*}
%Plugging in $L_2$ and doing some algebra, we get that the constant is
%\[L_3=\alpha^3L_u(L_x(1+\gamma))^2+3\alpha^2L_x(1+\gamma)L_u+ 3\alpha L_u+R\]
%Continuing in this fashion we can derive that
%\begin{align*}
%    L_4=&\alpha^4L_u(L_x(1+\gamma))^3+4\alpha^3L_u(L_x(1+\gamma))^2\\
%    &+4L_u\alpha^2L_x(1+\gamma)L_u+4\alpha
%    L_u+R\end{align*}
%and so on so that
%\begin{align*}
%    L_k=R+\alpha^kL_u(L_x(1+\gamma))^{k-1}+kL_u\sum_{i=1}^{k-1}
%    \alpha^i(L_x(1+\gamma))^{i-1}
%\end{align*}
%\end{proof}
%
%Then, we are interested in bounding $\|TQ_t(\theta)-TQ_t(\theta')\|$. Indeed,
%%    Consider the term
%%\[\alpha\mb{E}_{x',w}[\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta)+\tilde{v}(y(\theta'),\theta)-\tilde{
%%\uv}(y(\theta'),\theta')]\]
%   \begin{align*}
%        \|TQ_t(\theta)-TQ_t(\theta')\|
%        &\leq\alpha\|\mb{E}_{x',w}[\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta)]\|\\
%            &\ \ +\alpha\|\mb{E}_{x',w}[\tilde{v}(y(\theta'),\theta)-\tilde{
%        \uv}(y(\theta'),\theta')]\|\\
%        &\ \ +\|Q_t(\theta)-Q_t(\theta')\|
%    \end{align*}
%%Now,
%%\begin{align*}
%%    &\|\mb{E}_{x',w}[\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta)]\|\\
%%    &\qquad=\sum_{x',w}\tilde{P}(x',w|x,a)\|(\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta))\|
%%\end{align*}
%%and 
%    Recall that $\tilde{v}$ is
%Lipschitz in $\theta$ so that, by a similar argument,
%\begin{align*}
%    &\|\mb{E}_{x',w}[\tilde{v}(y(\theta'),\theta)-\tilde{
%    \uv}(y(\theta'),\theta')]\\
%    &\qquad\leq \sum_{x',w}\tilde{P}(x',w|x,a)\|\tilde{v}(y(\theta'),\theta)-\tilde{
%    \uv}(y(\theta'),\theta')]\|\\
%    &\qquad \leq L_\theta\|\theta-\theta'\|
%\end{align*}
%since $\sum_{x',w}\tilde{P}(x',w|x,a) =1$.
%
%By assumption $\tilde{v}$ is Lipschitz in $y$ with constant $L_y(\theta)$ so
%that
%\begin{align*}
%    &\|\mb{E}_{x',w}[\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta)]\|\\
%    &\qquad=\sum_{x',w}\tilde{P}(x',w|x,a)\|(\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta))\|\\
%    &\qquad\leq \sum_{x',w}\tilde{P}(x',w|x,a) L_y\|y(\theta)-y(\theta')\|\\
%    &\qquad
%    =\sum_{x'}P(x'|x,a)L_y\|\gamma(g(x',\theta)-g(x',\theta'))+Q_t(\theta')-Q_t(\theta)\|\\
%    &\qquad\leq L_y(\gamma L_t\|\theta-\theta'\|+\|Q_t(\theta')-Q_t(\theta)\|)
%    %\leq
%    %L_y\|y(\theta)-y(\theta')\|
%\end{align*}
%   Hence,
%      \begin{align*}
%        \|TQ_t(\theta)-TQ_t(\theta')\|
%        &\leq\alpha\|\mb{E}_{x',w}[\tilde{v}(y(\theta),\theta)-\tilde{v}(y(\theta'),\theta)]\|\\
%            &\ \ +\alpha\|\mb{E}_{x',w}[\tilde{v}(y(\theta'),\theta)-\tilde{
%        \uv}(y(\theta'),\theta')]\|\\
%        &\ \ +\|Q_t(\theta)-Q_t(\theta')\|\\
%        &\leq \alpha (\gamma+1)L_y L_t\|\theta-\theta'\|+\alpha
%        L_\theta\|\theta-\theta'\|\\
%        &\qquad+L_t\|\theta-\theta'\|
%    \end{align*}
%
%

